Towards the non-perturbative cosmological bootstrap

We study quantum field theory on a de Sitter spacetime dS$_{d+1}$ background. Our main tool is the Hilbert space decomposition in irreducible unitary representations of its isometry group $SO(d+1,1)$. As the first application of the Hilbert space formalism, we recover the K\"allen-Lehmann spectral decomposition of the scalar bulk two-point function. In the process, we exhibit a relation between poles in the corresponding spectral densities and the boundary CFT data. Moreover, we derive an inversion formula for the spectral density through analytical continuation from the sphere and use it to find the spectral decompisiton for a few examples. Next, we study the conformal partial wave decomposition of the four-point functions of boundary operators. These correlation functions are very similar to the ones of standard conformal field theory, but have different positivity properties that follow from unitarity in de Sitter. We conclude by proposing a non-perturbative conformal bootstrap approach to the study of these late-time four-point functions, and we illustrate our proposal with a concrete example for QFT in dS$_2$.

==> main/AdSTodS.tex <==
%!TEX root = ../QFTindS.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this appendix we collect various statements that deal with the relation between de Sitter space dS${}_{d+1}$ and Euclidean AdS$_{d+1}$ (or EAdS). This relation is fruitful because many interesting quantities, like correlation functions, can be computed rather easily in AdS. In what follows we present the recipe of analytical continuation and in-in formalism that is used to calculate contact and exchange tree level diagrams in dS. Many of the results presented below have appeared before, in particular in~\cite{Sleight:2019hfp,Sleight:2019mgd}. We reproduce them here for convenience, but refer to the original works for more details. 

In order to spell out the relation between dS and AdS, we recall that both of these spacetimes are defined as hypersurfaces living in the Minkowski space of $\mathcal{M}^{d+2}$:
\bsub
\begin{align}
& X_A X^A = -(X^{0})^2+(X^{1})^2+\ldots+(X^{d+1})^2 = R^2  && \text{dS}_{d+1}\\
& Y_A Y^A = -(Y^{0})^2+(Y^{1})^2+\ldots+(Y^{d+1})^2 = -R^2 && \text{EAdS}_{d+1}~.
\end{align}
\esub
Formally, passing from EAdS to dS amounts to setting $Y^A \to \pm i X^A$. The choice of the sign in this dictionary plays an important role for the analytical continuation in correlators that will appear below.

Poincar\'{e} coordinates for dS were defined in~\reef{Xetax}. For EAdS, these are defined as
\begin{equation}\label{PioncaredSAdS}
  Y^A=\frac{R}{z}\left(\frac{1+z^2+x^2}{2},x^\mu,\frac{1-z^2-x^2}{2}\right),
  \qquad
  x^\mu \in \mbb{R} \qaq z > 0~.
\end{equation}
The transformation $z\to\pm i\eta$ is the transformation that takes us from EAdS to dS. This choice of coordinates leads to metrics
\begin{equation}
ds^2_{\text{dS}} = R^2\, \frac{-d\eta^2+dx^2}{\eta^2}~, \qquad  ds^2_{\text{EAdS}} = R^2\, \frac{dz^2+dx^2}{z^2}~.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Two-point functions}

Two-point functions between points $X_1$, $X_2$ in dS or $Y_{1,2}$ in AdS can be expressed in terms of $SO(d+1,1)$ invariants
\bsub
\beq
\sigma_{\mrm{dS}} = \frac{1+X_1 \cdot X_2/R^2}{2} = 1 - \frac{(X-X')^2}{4R^2} \in \mbb{R}
\qaq
\sigma_{\mrm{AdS}} = \frac{1+Y_1 \cdot Y_2/R^2}{2} = - \frac{(Y-Y')^2}{4R^2} < 0
\eeq
or in coordinates~\cite[(2.13)]{Sleight:2019mgd}  
\beq
\sigma_{\text{dS}} = -\frac{|x_1-x_2|^2 - (\eta_1+\eta_2)^2}{4\eta_1\eta_2} 
\qaq
\sigma_{\text{AdS}}=-\frac{|x_1-x_2|^2+(z_1-z_2)^2}{4z_1 z_2}~.
\eeq
\esub
Since an analytic continuation needs to take $\sigma_{\mrm{AdS}}$ into $\sigma_{\mrm{dS}}$, it is clear that $z_1$ and $z_2$ must pick up an opposite phase:
\beq
\label{eq:conti}
(z_1,z_2) \mapsto (-i\eta_1,i \eta_2)
\quad\text{or}\quad
(i\eta_1,-i\eta_2)~.
\eeq
The dS propagator is given by the analytic continuation not of the AdS propagator, but of the AdS harmonic function $\Omega_{\nu}(Y_1,Y_2)$. This object is closely related to the AdS propagator: in fact, it appears in the split representation~\cite{Cornalba:2007zb, Costa:2014kfa} of the propagator.  The prescription~\reef{eq:conti} therefore provides two different methods to obtain a dS propagator. It turns out that the two continuations are not identical. In fact, the harmonic function $\Omega_{\nu}(Y_1,Y_2)$  has a branch cut starting at $\sigma = 1$, which is unphysical in AdS (since $\sigma_\mrm{AdS} < 0$) but corresponds to lightlike separated points in dS. The two prescriptions therefore give rise to two different dS propagators:~\cite[(2.23)]{Sleight:2019mgd}:
\beq
G(\sigma_\pm)
\quad
\text{where}
\quad
\sigma_{\pm} = 1 + \frac{ (\eta_1 - \eta_2 \pm i \epsilon)^2 - |x_1-x_2|^2}{4\eta_1\eta_2}~.
\eeq
The two different sign choices will play a role in the in-in formalism, which will be explained in the next section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{In-in formalism}

In the present section, we will briefly review the in-in formalism used in the computation of dS correlators. We will mostly refer to~\cite{Weinberg:2005vy}.
Recall that the flat-space S-matrix is related to correlation functions via LSZ reduction. There we assume cluster decomposition, meaning that in the far past (starting from a so-called ``in'' state)  and the far future (evolving towards an ``out'' state), the states can be written as the product of non-interacting single particle states. In particular, we assume that the vacuum is the free theory vacuum $\ket{0}$. In other words, we assume that we turn the interaction on and off adiabatically. In the case of dS, we still may ask to turn interactions on adiabatically, but correlation functions at late times (which are of interest to us) do not necessarily decompose into products free single-particle states. As such, there is no well-defined notion of ``out''-states.\footnote{One way to derive perturbation theory in QFT textbooks  makes use of the formula
\[
\bra{\Omega}T\{\phi(x) \phi(y)\} \ket{\Omega} = \lim_{T\to\infty(1-i\epsilon)}\frac{\bra{0}T\{\phi_I(x) \phi_I(y) e^{-i\int^\infty_{-\infty} dt H_I(t)}\} \ket{0}}{\bra{0} T\{e^{-i\int^\infty_{-\infty} dt H_I(t)} \} \ket{0}}
\]
where the $\ket{0}$ and $\ket{\Omega}$ are respectively the vacuum of the free theory and interacting theory. However, to derive this formula, one needs to assume that it is possible to evolve back $\ket{0}$ with a unitary operator $U(t,t^\prime)$ from $T\to +\infty$ to some $t^*=\max(x,y,t_{\text{integral}})$. This is not possible in dS.}

In the case of late-time correlators in dS, the in-out formalism cannot be used. Instead, to calculate the correlator
\[
\langle Q(t) \rangle=\langle \mathcal{O}(t,x_1)\mathcal{O}_2(t,x_2)\dotsm\mathcal{O}_n(t,x_n) \rangle
\]
at some time $t$ we use the \emph{in-in  formalism}, in which we evolve with a unitary operator from time $t_0=-\infty$ to $t$ and evolve back in time again to $t_0=-\infty$ as follows:
\begin{equation}\label{eq:In-in correlator}
\langle Q(t)\rangle = \langle \bar{T}\{e^{i\int_{t_0-i\epsilon}^{t-i\epsilon} dt^{\prime \prime} H_I(t^{\prime \prime})} \} Q_I(t) T\{e^{-i\int_{t_0+i\epsilon}^{t+i\epsilon} dt^\prime H_I(t^\prime)} \}\rangle
\end{equation} 
where the $T$ (resp.\@ $\bar{T}$) time-orders (anti-time-orders) operator produts, cf.\@ formula (1) from~\cite{Weinberg:2005vy}. 
Note that the $i \epsilon$ on the right hand side comes with plus sign while the one on the left has a minus sign. This has a convenient representation in the so-called Keldysh-Schwinger picture, where we have a branch cut on the real axis of the $t$-plane. To calculate the above correlator $\expec{Q(t)}$, we first evolve from $t=-\infty$ and move above the cut to $t$ (time ordered and $+i\epsilon$) and go back (anti-time ordered) from below the cut ($-i\epsilon$).

The prescription~\reef{eq:In-in correlator} results in a new set of Feynman rules, which are for instance explained in the appendix of~\cite{Weinberg:2005vy}. We review them here for completeness:
\begin{itemize}
\item Two different sets of vertices correspond to time-ordered and  anti-time-ordered terms. We call them right and left vertices, referring to their position in the operator product~\reef{eq:In-in correlator}. The right vertex gets multiplied by $-i$,  while the left vertex gets multiplied by $+i$.
\item The external propagator emanating from a right vertex and the propagator between two right vertices refer to the time-ordered propagator $\langle T\phi(x,t_1) \phi(y,t_2)\rangle$. %In the case of external operator we have $t=-\infty$.
\item Similarly, the external propagator leaving a left vertex and the propagator between two left vertices denotes the anti-time ordered propagator $\langle \bar{T} \phi(x,t_1) \phi(y,t_2)\rangle$.
\item The propagator between a right and a left vertex represents the Wightman function $\langle \phi(x,t_1) \phi(y,t_2)\rangle$.
\end{itemize}
Consequently, perturbation theory computations in dS make use of four different propagators involving two fields $\phi(x_1,t_1)$ and $\phi(x_2,t_2)$: 
\bsub
\beq
\label{eq:Gplusminus}
G_{-+}=G(\sigma_{-})=\langle \phi(x_1,t_1) \phi(x_2,t_2)\rangle ~, \qquad 
G_{+-}=G(\sigma_{+})=\langle \phi(x_2,t_2) \phi(x_1,t_1)\rangle~.
\eeq
The time-ordered and anti-time-ordered propagators are
\begin{align}
  \label{eq:Gplusplus}
  G_{++} &= \langle T\phi(x,t_1) \phi(y,t_2)\rangle = \theta (t_1-t_2) G_{-+} + \theta (t_2-t_1) G_{+-}~ \\
G_{--} &= \langle \bar{T}\phi(x,t_1) \phi(y,t_2)\rangle = \theta (t_1-t_2) G_{+-} + \theta (t_2-t_1) G_{-+}~.
\end{align}
\esub



==> main/constraints.tex <==
%!TEX root = ../HTinAdS.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter{Symmetry constraints on matrix elements}
\label{app:constraints}

In this appendix, we consider constraints coming from AdS isometries (or boundary conformal symmetry) on matrix elements of the operator
\beq
V \ldef R^{\DD_\mca{V}} \int_{-\pi/2}^{\pi/2} \!\frac{dr}{(\cos r)^2}\; \mca{V}(\tau=0,r)
\eeq
where $\mca{V}$ is any local bulk operator. To this end, we fix two boundary primary states $\ket{\psi_i}$ and $\ket{\psi_j}$ of dimension $\DD_i$ and  $\DD_j$. We will use ${SL}(2,\mbb{R})$ symmetry to derive relations between different matrix elements between descendants, that is to say between the matrix elements
\beq
\mbf{V}\ud{j,m}{i,n} \ldef \bbraket{\psi_j,m}{V}{\psi_i,n}.
\label{VmatelApp}
\eeq
The argument will make use of a second operator $W$, defined as follows:
\beq
W \ldef R^{\DD_\mca{V}}  \int_{-\pi/2}^{\pi/2} \frac{dr}{(\cos r)^2}\, \sin r\, \mca{V}(0,r)
\eeq
along with its matrix elements which we denote as $\mbf{W}\ud{j,m}{i,n}$ as in eq.~\reef{VmatelApp}. Parts of our discussion will be similar in spirit to section\@ 2.1 of reference~\cite{Fitzpatrick:2010zm}, where relations between matrix elements in AdS${}_3$ were derived using ${SO}(2,2)$ group theory.

\section{Relations between matrix elements of descendants}
\label{sec:relrelrel}

Let us proceed with the derivation of the promised relations. We derive them simply by evaluating Ward identities. If $G$ is a generator of ${SL}(2,\mbb{R})$, then $G \ket{\psi_i,n}$ can be computed using eq.~\reef{eq:KPonstates}. To wit
\bsub
\begin{align}
H \ket{\psi_i,n} &= (\DD_i + n) \ket{\psi_i,n},\\
K \ket{\psi_i,n} &= \gamma(\DD_i,n) \ket{\psi_i,n-1},\\
P \ket{\psi_i,n} &= \gamma(\DD_i,n+1) \ket{\psi_i,n+1}
\end{align}
\esub
where $\ga(\DD,n) = \sqrt{n(2\DD+n-1)}$. At the same time, $G$ acts on the local operators $\mca{V}$ as a differential operator $\mca{D}_G$, as specified in Eq.~\reef{eq:genAct}.
For general $G$, we then  have the identity
\bsub
\begin{align}
\bbraket{\psi_j,m}{[G,\mca{V}(\tau,r)]}{\psi_i,n} &= \mca{D}_G \cdot \bbraket{\psi_j,m}{\mca{V}(\tau,r)}{\psi_i,n}\\
&= (\bra{\psi_j,m}G) \mca{V}(\tau,r) \ket{\psi_i,n} - \bra{\psi_j,m} \mca{V}(\tau,r) (G \ket{\psi_i,n}).
\end{align}
\esub
For $G = H$, this implies that
\beq
\label{eq:Drell}
\left(\frac{\pd}{\pd \tau} + \DD_{ij} + n-m \right)\!  \bbraket{\psi_j,m}{\mca{V}(\tau,r)}{\psi_i,n} = 0
\eeq
where $\DD_{ij} \ldef \DD_i - \DD_j$. This completely fixes the $\tau$-dependence of $\bbraket{\psi_j,m}{\mca{V}(\tau,r)}{\psi_i,n}$. Likewise, for $P$ we get
\begin{multline}
\label{eq:Prell}
\mca{D}_P \cdot \bbraket{\psi_j,m}{\mca{V}(\tau,r)}{\psi_i,n} = \ga(\DD_j,m) \bbraket{\psi_j,m-1}{\mca{V}(\tau,r)}{\psi_i,n}\\ - \ga(\DD_i,n+1)  \bbraket{\psi_j,m}{\mca{V}(\tau,r)}{\psi_i,n+1}
\end{multline}
and finally for $K$ we have
\begin{multline}
\label{eq:Krell}
\mca{D}_K \cdot \bbraket{\psi_j,m}{\mca{V}(\tau,r)}{\psi_i,n} = \ga(\DD_j,m+1) \bbraket{\psi_j,m+1}{\mca{V}(\tau,r)}{\psi_i,n}\\ - \ga(\DD_i,n)  \bbraket{\psi_j,m}{\mca{V}(\tau,r)}{\psi_i,n-1}.
\end{multline}
To proceed, we explicitly apply the operators $\mca{D}_{P}$ and $\mca{D}_K$, which are first order both in $\pd_\tau$ and $\pd_r$. The $\tau$-derivatives can be computed by means of~\reef{eq:Drell}. The LHS of~\reef{eq:Prell} then becomes
\beq
(\ldots) = \left[(-\DD_{ij} + m -n) \sin r + \cos r\, \frac{\pd}{\pd r} \right]\!\bbraket{\psi_j,m}{\mca{V}(0,r)}{\psi_i,n}
\eeq
setting $\tau = 0$ from now on. The $\sin r$ term can be integrated over $r$ yielding something proportional to the matrix element $\mbf{W}\ud{j;m}{i;n}$. The second term can be computed similarly after employing integration by parts:
\bsub
\begin{align}
\int_{-\pi/2}^{\pi/2} \frac{dr}{(\cos r)^2} \cos r\, \frac{\pd}{\pd r} \bbraket{\psi_j,m}{\mca{V}(0,r)}{\psi_i,n} &= - \int_{-\pi/2}^{\pi/2} \frac{dr}{(\cos r)^2}  \sin r\,  \bbraket{\psi_j,m}{\mca{V}(0,r)}{\psi_i,n}\\
&= - \mbf{W}\ud{j;m}{i;n}
\end{align}
\esub
discarding a boundary term that vanishes. Integrating the RHS of~\reef{eq:Prell} at $\tau = 0$ as well, we obtain the relation
\bsub
\label{eq:VWrels}
\beq
(-\DD_{ij} + m-n-1) \mbf{W}\ud{j;m}{i;n} = \gamma(\DD_j,m) \mbf{V}\ud{j;m-1}{i;n} - \gamma(\DD_i,n+1) \mbf{V}\ud{j;m}{i;n+1}.
\eeq
If we repeat this for $K$, we get in addition
\beq
(-\DD_{ij} + m-n+1) \mbf{W}\ud{j;m}{i;n} = \gamma(\DD_j,m+1) \mbf{V}\ud{j;m+1}{i;n} - \gamma(\DD_i,n) \mbf{V}\ud{j;m}{i;n-1}.
\eeq
\esub
Moreover, matrix elements with either $n=0$ or $m=0$ can be computed as definite integrals over
\beq
f_{ji}(r) \ldef  \bbraket{\psi_j}{\mca{V}(0,r)}{\psi_i}
\eeq
which only involves the primary states $\ket{\psi_{i,j}}$. To wit:
\bsub
\label{eq:VWedge}
\begin{align}
  \label{eq:Vexp}
 \mbf{V}\ud{j;m}{i;0} &= (-1)^m \sqrt{\frac{m!}{(2\DD_j)_m}}  \int_{-\pi/2}^{\pi/2}\!\frac{dr}{(\cos r)^2} \, C_m^{-\half(m-\DD_{ij} )}(\sin r)  f_{ji}(r),\\
 \mbf{W}\ud{j;m}{i;0} &=  (-1)^{m+1} (m+1) \sqrt{\frac{m!}{(2\DD_j)_m}}  \int_{-\pi/2}^{\pi/2}\!\frac{dr}{(\cos r)^2} \, \frac{C_{m+1}^{-\half(m-\DD_{ij}+1 )}(\sin r)}{m-\DD_{ij}+1} \, f_{ji}(r).
\end{align}
\esub
Here $C_n^{(\nu)}(\cdot)$ denotes a Gegenbauer polynomial. Matrix elements with $m=0$ but $n \neq 0$ can be computed similarly, exchanging $\DD_i \lra \DD_j$ in the above formulas. In order to derive~\reef{eq:VWedge}, let
\beq
\mca{F}_m(r) \ldef \bbraket{\psi_j,m}{\mca{V}(0,r)}{\psi_i}
\eeq
omitting labels for the external states $\ket{\psi_{i,j}}$, and in particular $\mca{F}_0(r) = f_{ji}(r)$. Setting $n=0$ in~\reef{eq:Krell}, we get the recurrence relation
\beq
 \mca{F}_{m+1}(r) = \frac{1}{\ga(\DD_j,m+1)} \left[(-\DD_{ij} + m) \sin r - \cos r \, \frac{\pd}{\pd r} \right]\!\mca{F}_m(r).
\eeq
After repeatedly integrating by parts and discarding (vanishing) boundary terms, the formulas~\reef{eq:VWedge} are recovered.

The interpretation of the above results depends on the precise value of $\DD_{ij} = \DD_i - \DD_j$. We will discuss the cases where $\DD_{ij}$ is fractional and integer separately:
\begin{itemize}
\item If $\DD_{ij}$ is non-integer, the relations~\reef{eq:VWrels} together with the ``initial conditions''~\reef{eq:VWedge} are sufficient to compute \emph{any} matrix element of $\mbf{V}$. This can be done simply by eliminating $\mbf{W}$ from the equations~\reef{eq:VWrels}.
\item 
On the other hand, if $\DD_{ij}$ is an integer, it is not always possible to eliminate ${\mbf{W}}$ from the above equations. Instead, we find \emph{new} relations between specific matrix elements:
\bsub
\begin{align}
  \ga(\DD_j,m+1)\mbf{W}\ud{j;m+1}{i;m-\DD_{ij}} &= \ga(\DD_i,m-\DD_{ij})\mbf{W}\ud{j;m}{i;m-\DD_{ij}-1} + \mbf{V}\ud{j;m}{i;m-\DD_{ij}},\\
  \ga(\DD_i,m+1) \mbf{W}\ud{j;m+\DD_{ij}}{i;m+1} &= \gamma(\DD_j,m+\dd_{ij}) \mbf{W}\ud{j;m+\DD_{ij}-1}{i;m} + \mbf{V}\ud{j;m+\DD_{ij}}{i;m}
\end{align}
\esub
which are once more derived by a judicious application of integration by parts. It turns out that these identities are again sufficient to reduce the computation of the matrix $\mbf{V}$ to its boundary.
\end{itemize}

If $\DD_{ij}$ is integer, certain selection rules apply. For concreteness, consider the case $\DD_i = \DD_j$. Then by setting $m=n+1$ in the first relation of~\reef{eq:VWrels}, we obtain the identity
\beq
0 = \ga(\DD_i,n+1) \mbf{V}\ud{j;n}{i;n} - \ga(\DD_i,n+1) \mbf{V}\ud{i;n+1}{i;n+1}
\eeq
which implies that all matrix elements $\mbf{V}\ud{j;n}{i;n}$ with $n=0,1,2,\ldots$ are identical. This result has a simple physical meaning. Indeed, if $\psi_j = \psi_i$, the diagonal of the matrix $\mbf{V}\ud{i;n}{i;n}$  is proportional to the tree-level energy shift of the states $\ket{\psi_i,n}$. But by conformal symmetry, all such energy shifts (or anomalous dimensions) must be identical. Consequently, it is necessary that for $\DD_i = \DD_j$, the diagonal of the matrix $\mbf{V}$ is constant. 

Next, consider the case where $\DD_{ij}$ is a non-zero integer, say $\DD_{ij} \rdef s$ with $s \in \{1,2,3,\ldots\}$. Then from~\reef{eq:Vexp} it follows that $\mbf{V}\ud{j;s}{i;0}$ vanishes --- this is simply a property of the Gegenbauer polynomials. But from Eq.~\reef{eq:VWrels} it follows that
\beq
\ga(\DD_j,n+s+1) \mbf{V}\ud{j;n+s+1}{i;n+1} = \ga(\DD_i,n+1) \mbf{V}\ud{j;n+s}{i;n}
\eeq
for any $n$. Consequently, \emph{all} matrix elements of the form $\mbf{V}\ud{j;n+s}{i;n}$ vanish! If $\DD_{ij}$ is a negative integer, a similar argument can be made.

Let us finally comment on parity. If $\ket{\psi_{i,j}}$ have the same parity and $\mca{V}$ respects parity, then $f_{ji}(r)$ is even under $r \mapsto -r$. But then using~\reef{eq:VWedge} and~\reef{eq:VWrels}, it can be shown that matrix elements of $\mbf{V}$ (resp.\@ $\mbf{W}$) vanish if $m+n$ is odd (resp.\@ even). The same result could have been derived directly since
\beq
\bbraket{\psi_i,m}{\mtt{P}V\mtt{P}^{-1}}{\psi_j,n} = (-1)^{m+n}\bbraket{\psi_i,m}{V}{\psi_j,n} = + \bbraket{\psi_i,m}{V}{\psi_j,n}
\eeq
(using the fact that $\mtt{P}V\mtt{P}^{-1} = +V$) which for odd $m+n$ is only possible if $\mbf{V}\ud{j;m}{i;n} = 0$. A similar argument can be applied to the case where $\ket{\psi_{i,j}}$ have opposite parity.

\section{Example: vacuum amplitudes}

As an application of the above formalism, let's consider the case where the in-state is the vacuum $\ket{\Omega}$. By ${SL}(2,\mbb{R})$ symmetry, the wavefunction $f_{i,\Omega}$ is completely fixed, up to an overall constant:
\beq
f_{i,\Omega}(r) = \bbraket{\psi_i}{\mca{V}(r)}{\Omega} =  \a_i (\cos r)^{\DD_i}.
\eeq
The coefficient $\a_i$ can be interpreted as the bulk-boundary OPE coefficient of $\mca{V} \to \Oo_i$ (up to a convention-dependent constant), see~\reef{bulkToBound}. A short computation shows that
\beq
\mbf{V}\ud{i;2n+1}{\Omega} = 0,
\quad
\mbf{V}\ud{i;2n}{\Omega} = \a_i (\DD_i+2n)B(\th \DD_i - \th,\tfrac{3}{2})\sqrt{\frac{(\th)_n(\DD_i)_n}{n!(\DD_i+\th)_n}}
\eeq
where $B$ is the beta function. As an application of this result, we note that
\beq
\lim_{n \to \infty} \frac{\mbf{V}\ud{i;2n}{\Omega}}{\sqrt{n} \, \mbf{V}\ud{i;0}{\Omega}} = \frac{2}{\DD \sqrt{B(\th,\DD)}}
\eeq
that is to say that the matrix elements $\mbf{V}\ud{i;2n}{\Omega}$ grow as $\sqrt{n}$ at large $n$. In particular, this result implies that the Casimir energy diverges at least linearly at second order in perturbation theory. 


\section{Universality of matrix elements if $\DD_i - \DD_j$ is an even integer}
\label{subsec:constraintsEven}

If $\DD_{ij}$ is an even integer, that is to say $|\DD_i - \DD_j| = 2s$ for some integer $s$, and the in- and out-states $\ket{\psi_{i,j}}$ have the same parity, the matrix $\mbf{V}\ud{j;m}{i;n}$ is severely constrained. In fact, we will prove that it is fixed in terms of $s+1$ constants.

{\bf Theorem}: let $\ket{\psi_{i,j}}$ be two primaries with $\pi_i = \pi_j$ that satisfy $\DD_j = \DD_i \pm 2 s$ with $s \in \{0,1,2,\ldots\}$, and let $V$ be a parity-preserving bulk perturbation. Then the matrix ${\bf V}\ud{j;m}{i;n}$ 
is completely fixed by ${SL}(2,\mbb{R})$ symmetry in terms of the $s+1$ constants
\beq
c_a(\psi_j,\psi_i) \ldef \int_{-\pi/2}^{\pi/2}\!\frac{dr}{(\cos r)^2}\, (\sin r)^{2a} f_{ji}(r),
\quad
a = 0,1,\ldots,s.
\eeq
{\it Proof}: by parity, only matrix elements with even $m+n$ can be non-zero. Thus all non-vanishing matrix elements with $n=0$ are proportional to the following integral:
\[
\mbf{V}\ud{j;2m}{i;0} \; \propto \; \int_{-\pi/2}^{\pi/2}\!\frac{dr}{(\cos r)^2}\,  C_{2m}^{-m\pm s}(\sin r) f_{ji}(r),
\quad
m = 0,1,2,\ldots
\]
as an immediate consequence of~\reef{eq:VWedge}.  But it's easy to show that any such Gegenbauer polynomial is a polynomial of degree  $\leq s$ in the variable $z = (\sin r)^2$. Indeed, we have
\beq
\label{eq:functionsGalore}
C_{2m}^{-m + s}(\sin r) = \frac{(1-s)_m }{m!}\, {}_2F_1(-m,s,\th,z),
\quad
C_{2m}^{-m-s}(\sin r) = \frac{(1+s)_m}{m!}\, {}_2F_1(-s,-m,\th,z).
\eeq
The first of these functions vanishes if $m \geq s$, due to the prefactor $(1-s)_m$; for $m<s$ it's indeed a polynomial of degree $m$ in the variable $z$. 
Likewise, the second function in~\reef{eq:functionsGalore} is a polynomial in $z$ of degree $\text{min}(m,s)$. Consequently, any matrix element with $n=0$ can be expressed in terms of the parameters $c_a(\psi_j,\psi_i)$.

Now, the same argument can be applied to matrix elements with $m=0$. Finally, all other matrix elements, having $m,n \neq 0$ can be computed in terms of the previous ones using the relations described in section~\ref{sec:relrelrel}.
\qed

In particular, for $s=0$ (i.e.\@ whenever $\DD_i = \DD_j$) the matrix $\mbf{V}\ud{j;m}{i;n}$ is completely universal, meaning that it is fixed by symmetry up to an overall normalization. To be precise, we have the following corollary:

{\bf Corollary}: let $\ket{\psi_{i,j}}$ be two primaries with $\DD_i = \DD_j$ and $\pi_i = \pi_j$. Then for any parity-preserving bulk perturbation $V$, we have
\beq
\label{eq:eckhart}
\bbraket{\psi_j,m}{V}{\psi_i,n} = \msc{V}_{mn}(\DD_i) \, \bbraket{\psi_j}{V}{\psi_i}
\eeq
where $\msc{V}_{mn}(\DD_i)$ is a matrix that only depends on $\DD_i$, to wit:
\beq
\label{eq:Vmat}
\msc{V}_{mn}(\DD) = \begin{cases} 0 & \text{if } m + n \text{ is odd}; \\
  \sqrt{(m+1)_{n-m}/(2\DD+m)_{n-m}} &  m \leq n,\; m+n \text{ even}; \\
  \msc{V}_{nm}(\DD) & m > n.
\end{cases}
\eeq
{\it Note}: setting $m=n$, we see that the diagonal matrix elements are constant (since $\msc{V}_{nn}(\DD) = 1$). This is consistent with the discussion from the end of section~\ref{sec:relrelrel}.\\
{\it Proof}. Since any possible solution to the Ward identities is unique in this case, it suffices to check that $\msc{V}_{mn}(\DD_i)$ solves~\reef{eq:VWrels}. Indeed~\reef{eq:Vmat} is a valid solution, if we also have
\bsub
\beq
\bbraket{\psi_j,m}{W}{\psi_i,n} = \msc{W}_{mn}(\DD_i) \, \bbraket{\psi_j}{V}{\psi_i}
\eeq for
     \beq
     \msc{W}_{mn}(\DD)= \begin{cases} 0 & \text{if } m + n \text{ is even}; \\
   \sqrt{(m+1)_{n-m}/(2\DD+m)_{n-m}} &  m < n,\; m+n \text{ odd}; \\
   \msc{W}_{nm}(\DD) & m > n.
     \end{cases} 
     \eeq
     \esub
This can be checked easily.\qed


